The Reasoning-Memorization Interplay in Language Models Is Mediated by a Single Direction

Large language models (LLMs) excel on a variety of reasoning benchmarks, but previous studies suggest they sometimes struggle to generalize to unseen questions, potentially due to over-reliance on memorized training examples. However, the precise conditions under which LLMs switch between reasoning and memorization during text generation remain unclear. In this work, we provide a mechanistic understanding of LLMs' reasoning-memorization dynamics by identifying a set of linear features in the model's residual stream that govern the balance between genuine reasoning and memory recall. These features not only distinguish reasoning tasks from memory-intensive ones but can also be manipulated to causally influence model performance on reasoning tasks. Additionally, we show that intervening in these reasoning features helps the model more accurately activate the most relevant problem-solving capabilities during answer generation. Our findings offer new insights into the underlying mechanisms of reasoning and memory in LLMs and pave the way for the development of more robust and interpretable generative AI systems.

==> paper/5_application.tex <==
\section{Applications of LiReFs}
\label{sec:applications}
% \subsection{Improving LLM reasoning via LiReF intervention}


\subsection{Dataset Contamination Detection}



% they are some other dataset contamination detection methods... such as xx \citep{shi2023detecting} 

In Sections \ref{sec: cases analysis} and \ref{sec: reasoning generalization}, we observe that for certain reasoning problem samples, the model tends to rely more on its memory to provide answers and responses, and its performance on these samples lacks generalization. This suggests that the data from these downstream tasks might have leaked into the model's extensive pretraining corpus \citep{}. This undoubtedly affects the evaluation of the model's true capabilities, as the model is likely relying on replicating its memorized content to perform well on complex ability tests \citep{}. This leads us to consider whether the Linear Reasoning Features we extracted, along with the reasoning and memory feature regions we identified, can serve as a simple means of detecting such data contamination phenomena in the model.

% 接着讲data contanimination已经是一个研究很多的area，然后我们的方法跟其他人的方法在 wikimia，xxx上，在xxx，xxx ，xxx模型上跟这些方法做比较 or 提升


% 由于我们报告AUC分数作为评估指标，我们不需要确定阈值ϵ。


% 这些方法都是基于生成的token的概率分布，而我们的方法是基于实际的表征空间，模型内部完成任务所使用能力的倾向，因此可能有更好的互补性


% 还要解释为什么不能用新模型，因为benchmark的原因




\begin{table*}[ht]
\centering
% \footnotesize
\begin{tabular}{lccccc}
\toprule
\textbf{Method} & \textbf{BoolQ} & \textbf{Commonsense QA} & \textbf{IMDB} & \textbf{Truthful QA} & \textbf{Avg.} \\
\midrule
Neighbor & 0.68 & 0.56 & 0.80 & 0.59 & 0.66 \\
Zlib & 0.76 & 0.63 & 0.71 & 0.63 & 0.68 \\
Lowercase & 0.74 & 0.61 & 0.79 & 0.56 & 0.68 \\
PPL & 0.89 & 0.78 & 0.97 & 0.71 & 0.84 \\
\textsc{Min-k\% Prob} & \textbf{0.91} & \textbf{0.80} & \textbf{0.98} & \textbf{0.74} & \textbf{0.86} \\
\bottomrule
\end{tabular}
\caption{Example only. }
\label{tab:dataset_contamination}
\end{table*}

% \subsection{Detecting and mitigating reasoning data contamination}
